HFODD (v2.08k): User's Guide

We describe the input data and installation procedures of the code HFODD (v2.08k). The present write-up contains complete and comprehensive information that has originally been given in five independent publications. It is enhanced by the subject index and indexes of variables, input-data keywords, subroutines, and files that are used in this user guide.

==> index_of_files.tex <==
\begin{theindex}
    \input{index_header.tex}

  \item \textcolor{magenta}  {dy152-a.dat}, 50, 51, 57
  \item \textcolor{magenta}  {dy152-a.out}, 50
  \item \textcolor{magenta}  {dy152-b.dat}, 50, 51, 58
  \item \textcolor{magenta}  {dy152-b.out}, 50
  \item \textcolor{magenta}  {dy152-c.dat}, 50, 51, 61
  \item \textcolor{magenta}  {dy152-c.out}, 50
  \item \textcolor{magenta}  {dy152-d.dat}, 50, 51, 64
  \item \textcolor{magenta}  {dy152-d.out}, 50
  \item \textcolor{magenta}  {dy152-e.dat}, 50, 51, 65
  \item \textcolor{magenta}  {dy152-e.out}, 50
  \item \textcolor{magenta}  {dy152e-dat}, 51

  \indexspace

  \item \textcolor{magenta}  {hfodd.f}, 47, 49

  \indexspace

  \item \textcolor{magenta}  {la132-a.dat}, 50, 53, 55, 82
  \item \textcolor{magenta}  {la132-a.out}, 50
  \item \textcolor{magenta}  {la132-b.dat}, 50, 53, 55, 84
  \item \textcolor{magenta}  {la132-b.out}, 50

  \indexspace

  \item \textcolor{magenta}  {pb128-a.dat}, 50
  \item \textcolor{magenta}  {pb208-a.dat}, 55, 86
  \item \textcolor{magenta}  {pb208-a.out}, 50

  \indexspace

  \item \textcolor{magenta}  {sn120-a.dat}, 50, 56, 88
  \item \textcolor{magenta}  {sn120-a.out}, 50

  \indexspace

  \item \textcolor{magenta}  {tb-151-d.dat}, 53
  \item \textcolor{magenta}  {tb151-a.dat}, 50, 52, 53, 70
  \item \textcolor{magenta}  {tb151-a.out}, 50
  \item \textcolor{magenta}  {tb151-b.dat}, 50, 53, 73
  \item \textcolor{magenta}  {tb151-b.out}, 50
  \item \textcolor{magenta}  {tb151-c.dat}, 50, 53, 76
  \item \textcolor{magenta}  {tb151-c.out}, 50
  \item \textcolor{magenta}  {tb151-d.dat}, 50, 52, 79
  \item \textcolor{magenta}  {tb151-d.out}, 50

\end{theindex}


==> index_of_keywords.tex <==
\begin{theindex}
    \input{index_header.tex}

  \item \textcolor{blue}   {ALL\_DONE}, 7

  \indexspace

  \item \textcolor{blue}   {BASIS\_SIZE}, 32, 47

  \indexspace

  \item \textcolor{blue}   {CHAOTIC}, 11
  \item \textcolor{blue}   {CONT\_OMEGA}, 42
  \item \textcolor{blue}   {CONT\_PAIRI}, 42
  \item \textcolor{blue}   {COULOMB}, 30
  \item \textcolor{blue}   {COULOMFILE}, 40
  \item \textcolor{blue}   {COULOMSAVE}, 40
  \item \textcolor{blue}   {CUTOFF}, 18

  \indexspace

  \item \textcolor{blue}   {DIANON\_NEU}, 22
  \item \textcolor{blue}   {DIANON\_PRO}, 22
  \item \textcolor{blue}   {DIAPAR\_NEU}, 22, 26
  \item \textcolor{blue}   {DIAPAR\_PRO}, 27
  \item \textcolor{blue}   {DIASIG\_NEU}, 29
  \item \textcolor{blue}   {DIASIG\_PRO}, 29
  \item \textcolor{blue}   {DIASIM\_NEU}, 24
  \item \textcolor{blue}   {DIASIM\_PRO}, 24

  \indexspace

  \item \textcolor{blue}   {EALLMINMAX}, 38
  \item \textcolor{blue}   {EPS\_HERMIT}, 31
  \item \textcolor{blue}   {EQUASI\_MAX}, 38
  \item \textcolor{blue}   {EVE\_SCA\_PM}, 15
  \item \textcolor{blue}   {EVE\_SCA\_TS}, 14, 45
  \item \textcolor{blue}   {EXECUTE}, 7, 8, 39, 50, 51

  \indexspace

  \item \textcolor{blue}   {FIXDELTA\_N}, 16
  \item \textcolor{blue}   {FIXDELTA\_P}, 17

  \indexspace

  \item \textcolor{blue}   {G\_SCALING}, 16
  \item \textcolor{blue}   {GAUSHERMIT}, 31, 47

  \indexspace

  \item \textcolor{blue}   {HBAR2OVR2M}, 13
  \item \textcolor{blue}   {HFB}, 21
  \item \textcolor{blue}   {HOMEGAZERO}, 32

  \indexspace

  \item \textcolor{blue}   {INI\_DELTA}, 16
  \item \textcolor{blue}   {INI\_FERMI}, 16
  \item \textcolor{blue}   {ITERAT\_EPS}, 9
  \item \textcolor{blue}   {ITERATIONS}, 9

  \indexspace

  \item \textcolor{blue}   {LANDAU}, 13
  \item \textcolor{blue}   {LANDAU-SAT}, 14

  \indexspace

  \item \textcolor{blue}   {MAX\_MAGNET}, 30
  \item \textcolor{blue}   {MAX\_MULTIP}, 30
  \item \textcolor{blue}   {MAX\_SURFAC}, 30
  \item \textcolor{blue}   {MAXANTIOSC}, 9
  \item \textcolor{blue}   {MULTCONSTR}, 36

  \indexspace

  \item \textcolor{blue}   {NILSSONPAR}, 43
  \item \textcolor{blue}   {NUCLIDE}, 9

  \indexspace

  \item \textcolor{blue}   {ODD\_SCA\_PM}, 16
  \item \textcolor{blue}   {ODD\_SCA\_TS}, 15, 45
  \item \textcolor{blue}   {OMEGA\_RTP}, 34
  \item \textcolor{blue}   {OMEGA\_TURN}, 35
  \item \textcolor{blue}   {OMEGA\_XYZ}, 34, 42, 44
  \item \textcolor{blue}   {OMEGAY}, 34
  \item \textcolor{blue}   {OMISO\_XYZ}, 34
  \item \textcolor{blue}   {OMISOY}, 34
  \item \textcolor{blue}   {OPTI\_GAUSS}, 31, 44, 47

  \indexspace

  \item \textcolor{blue}   {PAIR\_FORCE}, 17
  \item \textcolor{blue}   {PAIR\_INTER}, 18
  \item \textcolor{blue}   {PAIRING}, 21
  \item \textcolor{blue}   {PAIRNFORCE}, 17
  \item \textcolor{blue}   {PAIRNINTER}, 17, 18
  \item \textcolor{blue}   {PAIRPFORCE}, 17
  \item \textcolor{blue}   {PAIRPINTER}, 18
  \item \textcolor{blue}   {PARITY}, 19
  \item \textcolor{blue}   {PHASESPACE}, 11, 47, 48
  \item \textcolor{blue}   {PHNONE\_NEU}, 22
  \item \textcolor{blue}   {PHNONE\_PRO}, 22
  \item \textcolor{blue}   {PHPARI\_NEU}, 25
  \item \textcolor{blue}   {PHPARI\_PRO}, 25
  \item \textcolor{blue}   {PHSIGN\_NEU}, 28
  \item \textcolor{blue}   {PHSIGN\_PRO}, 29
  \item \textcolor{blue}   {PHSIMP\_NEU}, 23
  \item \textcolor{blue}   {PHSIMP\_PRO}, 23
  \item \textcolor{blue}   {PING-PONG}, 10
  \item \textcolor{blue}   {PRINT-INTR}, 38
  \item \textcolor{blue}   {PRINT-ITER}, 38
  \item \textcolor{blue}   {PRINT-MOME}, 38

  \indexspace

  \item \textcolor{blue}   {READ\_WOODS}, 42
  \item \textcolor{blue}   {RECORDFILE}, 39
  \item \textcolor{blue}   {RECORDSAVE}, 40
  \item \textcolor{blue}   {REPLAYFILE}, 39
  \item \textcolor{blue}   {RESTART}, 42
  \item \textcolor{blue}   {REVIEW}, 39
  \item \textcolor{blue}   {REVIEWFILE}, 39
  \item \textcolor{blue}   {ROTATION}, 19

  \indexspace

  \item \textcolor{blue}   {SIGNATUREY}, 19
  \item \textcolor{blue}   {SIMPLEXY}, 19
  \item \textcolor{blue}   {SKYRME-SET}, 12
  \item \textcolor{blue}   {SKYRME-STD}, 12, 13, 44
  \item \textcolor{blue}   {SLOW-DOWN}, 30
  \item \textcolor{blue}   {SLOW-PAIR}, 16, 31
  \item \textcolor{blue}   {SPICON\_OME}, 35
  \item \textcolor{blue}   {SPICON\_XYZ}, 35
  \item \textcolor{blue}   {SPIN\_ORBIT}, 12, 13
  \item \textcolor{blue}   {SPINCONSTR}, 35
  \item \textcolor{blue}   {SURFAC\_DEF}, 32, 43
  \item \textcolor{blue}   {SURFAC\_PAR}, 32
  \item \textcolor{blue}   {SURFCONSTR}, 36

  \indexspace

  \item \textcolor{blue}   {TIMEREVERS}, 19
  \item \textcolor{blue}   {TSIMPLEX3D}, 21
  \item \textcolor{blue}   {TSIMPLEX\_Y}, 21
  \item \textcolor{blue}   {TSIMPLEXES}, 21

  \indexspace

  \item \textcolor{blue}   {VACPAR\_NEU}, 25
  \item \textcolor{blue}   {VACPAR\_PRO}, 25
  \item \textcolor{blue}   {VACSIG\_NEU}, 28
  \item \textcolor{blue}   {VACSIG\_PRO}, 28
  \item \textcolor{blue}   {VACSIM\_NEU}, 23
  \item \textcolor{blue}   {VACSIM\_PRO}, 23

  \indexspace

  \item \textcolor{blue}   {WOODSAFILE}, 40

\end{theindex}


==> index_of_subjects.tex <==
\begin{theindex}
    \input{index_header.tex}

  \item acronym, 12, 15, 45
  \item adiabatic, 50, 52, 53
  \item after variation, 13
  \item alignment, 26, 53
  \item angular frequency, 7, 19, 26, 34, 35, 42, 45, 51--55
  \item angular momentum, 26, 34, 35, 42, 45, 46, 53, 55
  \item average neutron pairing gap, 56

  \indexspace

  \item BCS blocking, 9
  \item BCS equation, 11, 16
  \item BCS pairing, 11, 19, 21, 34
  \item before variation, 13

  \indexspace

  \item canonical state, 11
  \item Cartesian axes, 46
  \item Cartesian components, 34
  \item Cartesian directions, 31, 32, 44, 47, 56
  \item center-of-mass, 12, 13, 44, 45
  \item chaotic, 11, 51
  \item charge block, 11
  \item charge--parity block, 25
  \item charge--parity--signature block, 28
  \item charge--simplex block, 11, 23, 55
  \item comment, 7, 44, 49
  \item compatibility, 19, 21, 35
  \item compiler, 48, 49
  \item conserved symmetries, 11, 51, 52
  \item constant potential, 16
  \item constraint, 30, 34--37, 46, 51, 54
  \item convergence, 9, 31, 44, 51, 53
  \item coordinate-space calculations, 56
  \item Coulomb direct energy, 46
  \item Coulomb direct potential, 40
  \item Coulomb exchange energy, 44, 46
  \item Coulomb field, 30, 40
  \item Coulomb file, 40, 41, 51
  \item Coulomb Green function, 30
  \item Coulomb interaction, 56
  \item coupling constant, 12, 14, 16, 44, 45
  \item CPU time, 19, 47--49, 51
  \item cranking term, 34
  \item crossing bands, 52
  \item cutoff energy, 11, 18, 32, 56

  \indexspace

  \item data line, 7, 8, 12, 39, 40
  \item data set, 7, 39, 46
  \item data value, 7
  \item default value, 7--12, 41, 50, 51
  \item deformation, 44, 45
  \item deformed harmonic oscillator, 32
  \item density matrices, 11, 18
  \item density-dependent part, 15
  \item density-dependent term, 56
  \item diabatic blocking, 11, 22, 24, 26, 27, 29, 50, 51
  \item diabatic-blocking data, 11
  \item diagonalization, 11, 55
  \item divergence, 10, 11, 51, 53--55
  \item doubly-magic nucleus, 55

  \indexspace

  \item eigenstate, 11, 55
  \item elementary charge, 44
  \item end of input data file, 7
  \item energy, 45
  \item energy density functional, 34, 36
  \item equivalent-spectrum, 56
  \item Euler angles, 45
  \item execution, 49

  \indexspace

  \item Fermi energy, 16, 56
  \item first iteration, 16, 42, 45, 55, 56
  \item form-factor, 17, 56

  \indexspace

  \item $g$-factor, 45
  \item Gauss-Hermite integration, 31, 47, 56
  \item Gauss-Hermite quadrature, 44
  \item generalized spin-orbit, 12, 13

  \indexspace

  \item Hermite polynomials, 31
  \item HFB calculations, 17, 56
  \item HFB equation, 21
  \item HFB pairing, 11, 16, 19, 21, 42
  \item HO basis, 32, 42--44, 47, 49, 51, 53, 56
  \item HO quanta, 44, 47
  \item HO state, 32, 47
  \item hole state, 11, 24, 26, 29

  \indexspace

  \item initial mean field, 9, 56
  \item input item, 7, 50, 51
  \item input parameter, 7, 41, 47, 50, 51, 55
  \item intrinsic frame, 38, 45, 46, 55
  \item intrinsic spin, 53, 56
  \item item, 7
  \item iteration, 9--11, 26, 30--32, 35, 38--40, 42, 44, 45, 51--56
  \item iteration number, 10

  \indexspace

  \item Kerman-Onishi condition, 55
  \item keyword line, 7, 8
  \item kinetic energy, 46
  \item kinetic-energy operator, 13

  \indexspace

  \item Landau parameters, 13
  \item linear momentum, 13

  \indexspace

  \item magic numbers, 55
  \item magnetic moment, 30, 38, 46
  \item mass, 44
  \item mass distribution, 54, 55
  \item mean-field Hamiltonian, 11
  \item memory, 47, 49
  \item mixing, 16, 31
  \item moment of inertia, 46
  \item multipole moment, 26, 30, 36, 38, 45

  \indexspace

  \item neutron skin, 56
  \item Nilsson asymptotic state, 45
  \item Nilsson labels, 46
  \item Nilsson potential, 9, 32, 43, 51--53, 56
  \item normalization factor, 36
  \item nuclear surface, 32, 44, 51
  \item number of iterations, 9
  \item number of neutrons, 11

  \indexspace

  \item occupied, 23, 25--28, 46, 53
  \item occupied state, 22, 23, 25, 55
  \item odd and odd-odd nuclei, 9
  \item odd or odd-odd nucleus, 19
  \item one-body center-of-mass, 13

  \indexspace

  \item pairing, 16--18, 21, 31, 46, 51--53, 55, 56
  \item pairing energy, 45, 46
  \item pairing gap, 16, 17, 46, 56
  \item pairing strength, 16
  \item pairing window, 11, 56
  \item parameter set, 12
  \item parity, 19, 25, 26, 28, 30, 45, 51--55
  \item parity block, 25, 46, 54, 55
  \item parity--signature block, 28, 29, 45, 46, 53, 54
  \item parity--signature configuration, 29, 55
  \item particle numbers, 9
  \item particle state, 11, 24, 26, 29
  \item particle-hole channel, 31
  \item particle-hole configuration, 11, 45
  \item particle-hole excitation, 22, 23, 25, 26, 28, 55
  \item particle-number symmetry, 56
  \item particle-particle channel, 56
  \item Pauli exclusion principle, 22, 23, 25
  \item phase space, 9
  \item ping-pong, 10, 11, 51, 53, 54
  \item planar solution, 53, 55
  \item principal axes, 32
  \item principal-axes frame, 45

  \indexspace

  \item quadrupole moment, 26, 45, 51, 54
  \item quasiparticle energies, 38
  \item quasiparticle properties, 38
  \item quasiparticle state, 18, 47, 56

  \indexspace

  \item radius, 45
  \item rearrangement energy, 46
  \item recommended value, 11, 50, 51
  \item record file, 39, 40, 42
  \item reference configuration, 22, 23, 25, 28
  \item replay file, 39, 42
  \item review file, 39
  \item root-mean-square radii, 56
  \item Routhian, 27, 38, 45, 46, 52, 53

  \indexspace

  \item saturation density, 17, 56
  \item self-consistent solution, 10, 55
  \item signature, 19, 28, 51--53
  \item simplex, 19, 21, 23, 24, 45, 51--53, 55
  \item simplex block, 24, 45, 46
  \item Simpson integration, 30
  \item single-particle configuration, 22, 52, 54
  \item single-particle energy, 9, 46
  \item single-particle observables, 10
  \item single-particle properties, 38, 39
  \item single-particle state, 23, 45, 47
  \item Skyrme force, 12--14, 44
  \item Skyrme functional, 9, 44, 45
  \item solid harmonics, 30
  \item spatial coordinates, 56
  \item spherical basis, 55, 56
  \item spherical code, 56
  \item spherical ground state, 55, 56
  \item spherical harmonics, 36
  \item spin, 26, 35, 45, 46
  \item spin-orbit, 12, 46
  \item stability, 9, 10, 46
  \item stability energy, 45
  \item standard FORTRAN input, 7
  \item standard FORTRAN output, 44
  \item starting point, 56
  \item superdeformed, 7, 50, 51
  \item surface multipole moment, 30, 36--38

  \indexspace

  \item tensor, 12
  \item termination of the HF iteration, 9
  \item theorem of self-consistent symmetries, 55
  \item tilted-axis-cranking, 50, 53
  \item time-even contribution, 45, 46
  \item time-even coupling constant, 15
  \item time-even potential, 31
  \item time-odd contribution, 45, 46
  \item time-odd coupling constant, 13, 15
  \item time-odd potential, 9, 31
  \item time-reversal, 19, 21, 51--53
  \item traditional spin-orbit, 12
  \item triaxial, 53--55
  \item two-body center-of-mass, 13

  \indexspace

  \item vector processor, 47

  \indexspace

  \item wave function, 11, 40
  \item Woods-Saxon file, 40, 42

  \indexspace

  \item zero-range density-dependent interaction,$\!$ 56
  \item zero-range density-dependent pairing,$\!$ 16, 17

\end{theindex}


==> index_of_subroutines.tex <==
\begin{theindex}
    \input{index_header.tex}

  \item \textcolor{green}  {CGEMM}, 48
  \item \textcolor{green}  {CPU\_TIME}, 49
  \item \textcolor{green}  {CPUTIM}, 49

  \indexspace

  \item \textcolor{green}  {DCLOCK}, 49

  \indexspace

  \item \textcolor{green}  {ETIME}, 49

  \indexspace

  \item \textcolor{green}  {F02AXE}, 48

  \indexspace

  \item \textcolor{green}  {GETTIM}, 49

  \indexspace

  \item \textcolor{green}  {PARAMS}, 12
  \item \textcolor{green}  {PREDEF}, 7

  \indexspace

  \item \textcolor{green}  {REVIEW}, 39

  \indexspace

  \item \textcolor{green}  {SETBAS}, 44

  \indexspace

  \item \textcolor{green}  {TIME}, 49

  \indexspace

  \item \textcolor{green}  {ZHPEV}, 48
  \item \textcolor{green}  {ZHPEVX}, 48

\end{theindex}

